SAILFISH: Vetting Smart Contract State-Inconsistency Bugs in Seconds

This paper presents SAILFISH, a scalable system for automatically finding state-inconsistency bugs in smart contracts. To make the analysis tractable, we introduce a hybrid approach that includes (i) a light-weight exploration phase that dramatically reduces the number of instructions to analyze, and (ii) a precise refinement phase based on symbolic evaluation guided by our novel value-summary analysis, which generates extra constraints to over-approximate the side effects of whole-program execution, thereby ensuring the precision of the symbolic evaluation. We developed a prototype of SAILFISH and evaluated its ability to detect two state-inconsistency flaws, viz., reentrancy and transaction order dependence (TOD) in Ethereum smart contracts. Further, we present detection rules for other kinds of smart contract flaws that SAILFISH can be extended to detect. Our experiments demonstrate the efficiency of our hybrid approach as well as the benefit of the value summary analysis. In particular, we show that S SAILFISH outperforms five state-of-the-art smart contract analyzers (SECURITY, MYTHRIL, OYENTE, SEREUM and VANDAL ) in terms of performance, and precision. In total, SAILFISH discovered 47 previously unknown vulnerable smart contracts out of 89,853 smart contracts from ETHERSCAN .

==> Makefile <==
# name of the tex file, without extension

FILENAME=sp
BIB = bibs/*.bib

all: sanitize $(FILENAME).tex
	rubber -Wall --unsafe --synctex --pdf $(FILENAME) || rubber -Wall --unsafe --synctex --pdf $(FILENAME)
	rubber-info $(FILENAME)
	xdg-open $(FILENAME).pdf	

clean:
	rubber --clean $(FILENAME)
	rm -f output/* *.log
	rm -f $(FILENAME).pdf

sanitize:
	sed -i 's/ i\.e\./ \\ie/g' sections/*.tex
	sed -i 's/ etc\./ \\etc/g' sections/*.tex
	sed -i 's/ viz\./ \\viz/g' sections/*.tex
	sed -i 's/ e\.g\./ \\eg/g' sections/*.tex

spellcheck:
	aspell check --lang=en_US $(FILENAME).tex

loop:
	while true; do inotifywait -r -e MODIFY $(SOURCES); printf %50s |tr " " "="; echo""; make clean; make;   done

check:
	chrisper *.tex

.PHONY: all clean clean_leavepdf spellcheck pdf loop check rtf

